Semifactual Explanations for Reinforcement Learning

Reinforcement Learning (RL) is a learning paradigm in which the agent learns from its environment through trial and error. Deep reinforcement learning (DRL) algorithms represent the agent's policies using neural networks, making their decisions difficult to interpret. Explaining the behaviour of DRL agents is necessary to advance user trust, increase engagement, and facilitate integration with real-life tasks. Semifactual explanations aim to explain an outcome by providing "even if" scenarios, such as "even if the car were moving twice as slowly, it would still have to swerve to avoid crashing". Semifactuals help users understand the effects of different factors on the outcome and support the optimisation of resources. While extensively studied in psychology and even utilised in supervised learning, semifactuals have not been used to explain the decisions of RL systems. In this work, we develop a first approach to generating semifactual explanations for RL agents. We start by defining five properties of desirable semifactual explanations in RL and then introducing SGRL-Rewind and SGRL-Advance, the first algorithms for generating semifactual explanations in RL. We evaluate the algorithms in two standard RL environments and find that they generate semifactuals that are easier to reach, represent the agent's policy better, and are more diverse compared to baselines. Lastly, we conduct and analyse a user study to assess the participant's perception of semifactual explanations of the agent's actions.

==> Res/JassDraftRelatedWork.tex <==
\section{Related Work}

Counterfactual explanations have been established as a powerful user-friendly explanation method in XAI. In RL, various approaches have been developed to generate counterfactual state explanations that can explain a specific action choice \cite{olson2021counterfactual,huber2023ganterfactual,gajcin2023raccer}. Additionally, counterfactual explanations providing sequences of actions that can be used to avoid a negative outcome have been explored \citep{gajcin2024acter,tsirtsis2021counterfactual,tsirtsis2023finding}.

Semifactuals are similar to counterfactuals in that they too imagine alternative worlds, however, semifactuals search for those in which the outcome did not change. For example, when explaining why a loan application was rejected, a semifactual might state that ”Even if your salary was twice as high, the application would still have been rejected. While counterfactual explanations can be used to understand how a negative outcome can be avoided, semifactuals could be utilized to optimize resources necessary for a positive outcome. For example, an AI system utilizing semifactuals could explain to the farmer that even if they used less fertilizer the yield would have remained the same. 

Methods for generating semifactuals in supervised learning can be classified into two groups -- counterfactually-free and counterfactually-guided methods. Counterfactually-guided approaches require a counter-
factual to be generated to guide the search for the semifactual. Intuitively, semifactuals are
often imagined between the original instance and the decision boundary. PIECE \cite{kenny2021generating} generates plausible counterfactuals in image-based tasks by identifying and resetting them to their expected values for the counterfactual class. A semifactual generation follows the same process except it terminates just before the decision boundary is reached. Counterfactually-free methods often rely on a metric to choose a semifactual that is the farthest away from the original instance. For example, \cite{nugent2009gaining} propose generating a neighborhood of instances around the original instance, and using logistic regression to classify. The semifactual is then chosen as the instance with the lowest probability of being classified as the original instance, which still belongs to that class. \cite{aryal2023even} propose MDN (Most Distant Neighbor) approach which searches for the semifactual as an instance that differs significantly from the original in one key feature. \cite{kenny2024utility} propose S-GEN, a method for generating semifactuals that relies on causality.
To generate semifactuals, authors start by creating a structural causal model (SCM) around the query
instance. Neighboring instances represent nodes, while actions that can transform one state
into another are actions. Achieving the semifactual means taking an action $a \in {a_1, ..., a_m}$ in the SCM. S-GEN then searches for the semifactual by optimizing three metrics -- gain, robustness and diversity. Gain depends on how distant two states are, as well as a predefined notion of what a favorable change is to the specific user. Robustness is measured in relation to instances in the neighborhood of the semifactual being classified into the same class. DIveristy encourages the generation of semifactuals with diverse features to enable personalization.

While explored in supervised learning, no approaches generate semifactual explanations for RL.
